Discovery and Multi-Wavelength Analysis of a New Dissociative Galaxy Merger: The Champagne Cluster

We report the discovery of a new binary galaxy cluster merger, the Champagne Cluster (RM J130558.9+263048.4), using a detection method that identifies dynamically active clusters in the redMaPPer SDSS DR8 photometric galaxy cluster catalog. The Champagne Cluster exhibits the classic X-ray morphology of a post-pericenter dissociative galaxy cluster merger: an X-ray peak located between two galaxy overdensities at the same redshift. We conducted a Keck/DEIMOS survey and obtained redshifts for {\bfseries 102} member galaxies. The redshift analysis indicates a relative velocity of 411 $\pm$ 180 km/s between the two subclusters, which suggests that the merger is happening near the plane of the sky. We estimated the bulk temperature (8.20 $\pm 1.2$ keV) and total X-ray luminosity (7.29 $\pm$ 0.19 $\times$ $10^{44}$ erg $\times$ $s^{-1}$) of the intracluster medium using $\textit{Chandra}$ archival data. We used the $\textit{ClusterPyXT}$ software to make a temperature map, and we compared it to hydrodynamic simulations to constrain the time since pericenter (TSP), the impact parameter, and the mass ratio. We found two scenarios that matched our data: a returning system with an impact parameter of 0 and TSP of 2.2 Gyr, and an outbound system with an impact parameter of 500 kpc and TSP of 0.4 Gyr. Both scenarios have a mass ratio of 1:10.

==> table2.tex <==
196.42445833 &26.46052778 & G & 0.3093\\
196.42479167 &26.51390278 & G & 0.30762\\
196.439875 &26.50904722 & G & 0.30397\\
196.44183333 &26.51400833 & G & 0.30943\\
196.45770833 &26.510725 & G & 0.31877\\
196.46208333 &26.49253611 & G & 0.30631\\
196.474875 &26.50268611 & G & 0.29772\\
196.477 &26.50217778 & G & 0.30946\\
196.47758333 &26.50889444 & G & 0.30981\\
196.482 &26.52460833 & G & 0.30796\\
196.48291667 &26.50816944 & G & 0.31752\\
196.48408333 &26.51236944 & G & 0.32331\\
196.486 &26.51475278 & G & 0.30591\\
196.48708333 &26.55572222 & G & 0.3096\\
196.502375 &26.51421389 & G & 0.31178\\
196.50504167 &26.51548611 & G & 0.30993\\
196.506625 &26.51511111 & G & 0.30314\\
196.516875 &26.54194444 & G & 0.29821\\
196.53008333 &26.5904 & G & 0.29849\\
196.535125 &26.54823333 & G & 0.30114\\
196.53641667 &26.51540556 & G & 0.31197\\
196.54291667 &26.554075 & G & 0.30463\\
196.55670833 &26.54493056 & G & 0.31005\\
196.56875 &26.57646667 & G & 0.30543\\
196.50284 &26.51781 & G & 0.3063\\
196.50683 &26.5155 & G & 0.302763\\
196.48232 &26.50952 & G & 0.320435\\
196.50708 &26.505 & G & 0.3063\\
196.5167 &26.51773 & G & 0.308148\\
196.47324 &26.52629 & G & 0.3063\\
196.46769 &26.55002 & G & 3.05356\\
196.4388 &26.48121 & G & 0.300674\\
196.56264 &26.46912 & G & 0.341063\\
196.41828 &26.48273 & G & 0.307494\\
196.4124 &26.48203 & G & 0.295\\
196.41239 &26.48202 & G & 0.295\\
